COLD: Towards the Next Generation of Pre-Ranking System

Multi-stage cascade architecture exists widely in many industrial systems such as recommender systems and online advertising, which often consists of sequential modules including matching, pre-ranking, ranking, etc. For a long time, it is believed pre-ranking is just a simplified version of the ranking module, considering the larger size of the candidate set to be ranked. Thus, efforts are made mostly on simplifying ranking model to handle the explosion of computing power for online inference. In this paper, we rethink the challenge of the pre-ranking system from an algorithm-system co-design view. Instead of saving computing power with restriction of model architecture which causes loss of model performance, here we design a new pre-ranking system by joint optimization of both the pre-ranking model and the computing power it costs. We name it COLD (Computing power cost-aware Online and Lightweight Deep pre-ranking system). COLD beats SOTA in three folds: (i) an arbitrary deep model with cross features can be applied in COLD under a constraint of controllable computing power cost. (ii) computing power cost is explicitly reduced by applying optimization tricks for inference acceleration. This further brings space for COLD to apply more complex deep models to reach better performance. (iii) COLD model works in an online learning and severing manner, bringing it excellent ability to handle the challenge of the data distribution shift. Meanwhile, the fully online pre-ranking system of COLD provides us with a flexible infrastructure that supports efficient new model developing and online A/B testing.Since 2019, COLD has been deployed in almost all products involving the pre-ranking module in the display advertising system in Alibaba, bringing significant improvements.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


==> experiment_old.tex <==
\section{Experiments}



We conducted experiments on COLD before it was deployed into our display advertising system. Specifically, we need to evaluate the offline performance, comparing COLD model with the previous ad pre-ranking ctr model and the current ranking ctr model. Then we need to conduct the online A/B test to evaluate the online performance.
\subsection{Competitors and Experiment Setup}
We compare COLD with the following baselines:
\begin{itemize}
        \item {\textbf{Vector-Product based DNN}} is the previous pre-ranking model in our display advertising system. The scores is calculated with inner products form between user embedding and ad embedding. 
        % \item {\textbf{COLD without Cross Features}} is the processed COLD model without cross features between user and ad.
        % \item {\textbf{COLD with more Cross Features}} is the processed COLD model with more cross features between user and ad.
        \item {\textbf{DIEN}} \cite{zhou2019dien}  is our previous version of ranking model. It integrates GRU with attention for capturing the evolution trend of user interests.      
\end{itemize}

\textbf{Experiment Settings.} 
COLD is trained  with more than 90 billion samples. Layers of FCN (Fully Connected Network) are set by $1024 \times 512 \times 256 \times 128 \times 64 \times 2$. The number of embedding dimension is set to be 16. we use Adam solver to update the model parameters. The GAUC \cite{zhou2018deep} is used as the metric to evaluate the offline performance of the models. The top k recall is also used to indicate the alignment degree between the pre-ranking model and the ranking model. 
\begin{equation}
  recall = \frac{|\{\text{top k ad canidates}\} \cap \{ \text{top m ad canidates}\}|}{|\{\text{top m ad canidates}\}\}|}.
\end{equation}
The top k ad candidates are ranked by the pre-ranking model and the top m ad candidates are ranked by ranking model. The ranking metric is cost per mile (CPM=CTR $\times$ Bid).

\subsection{Offline and Online Evaluation}

% The previous pre-ranking model in our display advertising system is a vector-product based model which makes inner products between user embedding and ad embedding. The two embeddings are calculated in an offline manner. The ranking model is DIEN \cite{zhou2019deep}. 

We conduct offline evaluation on the feed scenes in Taobao. As shown in Table \ref{exp:offline},  COLD  outperforms the vector-based model both in GAUC and recall. It also maintains a comparable result with DIEN.

The online A/B testing is also performed. As shown in Table \ref{exp:online}, the CTR of COLD increases 6.1\%\ and 9.1\%\ compared to the vector-product based model, which means that COLD can provide more accurate ads for users. The RPM also increases 6.5\%\ and 10.8\%\ which indicates the COLD method can bring more revenue for the Taobao display advertising platform. The results of COLD in double 11 event is better than normal, which proves that COLD can adapts to the newest data distribution when the data changes dramatically. 

% Two metrics are used to evaluate the performance:


% \begin{center}
% \begin{table}
% \begin{tabular}{ |c|c|c| } 
%  \hline
%  method & gauc & recall \\ 
%  \hline
%  vector based model & 0.6107 & 88\% \\ 
%   \hline
%  COLD & 0.6349 & 96\%\\ 
%  \hline
% DIEN & 0.6476 & 100\%\\ 
%  \hline
% \end{tabular}
% \caption{\label{tab:qps column computing}Offline Evaluation Results}
% \label{exp:offline}    
% \end{table}
% \end{center}


% \subsection{Online Evaluation}


% \begin{itemize}
% \item CTR = AdClickCount/AdPresentCount
% \item RPM = CTR $\times$ PPC
% \end{itemize} 



\begin{table}[t]
  \caption{Offline Evaluation Results}
\label{exp:offline}    
  \begin{tabular}{lcl}
    \toprule
     Method & GAUC & Recall\\
    \midrule
 Vector-based Model & 0.6107 & 88\% \\ 
%  COLD without Cross Features & 0.6250 & 91\%\\ 
 COLD & 0.6349 & 96\%\\ 
DIEN & 0.6476 & 100\%\\ 
  \bottomrule
\end{tabular}
\end{table}






\begin{table}
  \caption{Online Evaluation Results.}
\label{exp:online}    
  \begin{tabular}{lcl}
    \toprule
 Method & CTR & RPM \\ 
    \midrule
 Normal Days & +6.1\%\ & +6.5\%\ \\ 
 Double 11 Event& +9.1\%\ & +10.8\%\ \\ 
  \bottomrule
\end{tabular}
\end{table}

% 11.11：
% CTR：9.07
% RPM：10.79
% 11.7-11.9：
% CTR：6.10
% RPM：6.53




\subsection{Ablation Study}

We conduct experiments to evaluate the performance and computing power cost between different models and feature groups. The feature group candidates are selected by ranking results based on the importance weight of SE block.
We also conduct experiments to demonstrate the benefits of different optimization techniques. 

We first compare the system performance for different models, especially the vector-product based model, complicated ranking model, and COLD. Vector-product based model runs on a CPU machine with 2 Intel(R) Xeon(R) Platinum 8163 CPU @ 2.50GHz (96 cores) and 512GB RAM. Ranking model and COLD run on a GPU machine with NVIDIA T4 equipped. As shown in Table \ref{tab:qps}, the vector-based model has the lowest latency and highest throughput, while the ranking model is the opposite. Our COLD finds a nice balance between the two. 

\begin{table}
  \caption{The System Performance for Different Models}
\label{tab:qps}
  \begin{tabular}{lccc}
    \toprule
 Method & QPS & Latency & GAUC  \\ 
    \midrule
 Vector-based Model  & 100000 & 1ms & 0.6107 \\ 
 COLD with Less Features & 13000 & 6ms & 0.6250 \\ 
 COLD & 12000 & 7ms & 0.6349\\ 
 COLD with More Features & 10000 & 9ms & 0.6320 \\ 
DIEN & 1100 & 15ms & 0.6476\\ 
  \bottomrule
\end{tabular}
\end{table}


We then compare the row-based feature computation with the column-based method. We run our engine on a machine with 2 Intel(R) Xeon(R) Platinum 8163 CPU @ 2.50GHz (96 cores) and 512GB RAM. For each query, we set the batch size as 300. Table \ref{tab:rt_column} shows the running time for different stages of feature computation. As we can see, the column-based method accelerates the ad features computation by a factor of six. Table \ref{tab:qps_column} shows 
the throughput of the two methods. Column based method has only one-third of CPU load under the same QPS or obtains 3X throughput with similar CPU load.

\begin{table}
  \caption{The Run Time Performance}
\label{tab:rt_column}
  \begin{tabular}{cccc}
    \toprule
 Method & \makecell*[c]{User/Scene \\Features} & Ad Features & Post-Processing \\ 
    \midrule
 Row based & 0.49ms & 4.90ms & 0.75ms \\ 
 Column based & 0.40ms & 0.83ms & 0.49ms\\ 
  \bottomrule
\end{tabular}
\end{table}



% \begin{center}
% \begin{table}
% \begin{tabular}{ |c|c|c|c| } 
%  \hline
%  method & \makecell*[c]{user/scene \\features} & ad features & post-processing \\ 
%  \hline
%  row based & 0.49ms & 4.9ms & 0.75ms \\ 
%   \hline
%  column based & 0.40ms & 0.83ms & 0.49ms\\ 
%  \hline
% \end{tabular}
% \caption{\label{tab:rt column computing}Comparing the run time of different stages between row based computing column based computing. Batch size = 300}
% \end{table}
% \end{center}


% \begin{center}
% \begin{table}
% \begin{tabular}{ |c|c|c| } 
%  \hline
%  method & QPS & CPU load \\ 
%  \hline
%  row based & 3000 & 29\% \\ 
%   \hline
%  column based & 3000 & 10\%\\ 
%  \hline
% column based & 9000 & 33\%\\ 
%  \hline
% \end{tabular}
% \caption{\label{tab:qps column computing}Comparing the QPS (Query Per Second) and CPU load on single server between row based computing column based computing. Batch size = 300}
% \end{table}
% \end{center}


\begin{table}
  \caption{The QPS and CPU load Performance}
\label{tab:qps_column}
  \begin{tabular}{ccc}
    \toprule
 Method & QPS & CPU load \\ 
    \midrule
 Row based & 3000 & 29\% \\ 
 Column based & 3000 & 10\%\\ 
 Column based & 9000 & 33\%\\ 
  \bottomrule
\end{tabular}
\end{table}



% \begin{center}
% \begin{table}
% \begin{tabular}{ |c|c|c|c| } 
%  \hline
%  method & QPS & latency & gauc \\ 
%  \hline
%  vector based  & 100000 & 1ms & 0.62 \\ 
%   \hline
%  LDN & 12000 & 7ms & 0.65\\ 
%  \hline
% ranking model & 1100 & 15ms& 0.66\\ 
%  \hline
% \end{tabular}
% \caption{\label{tab:qps cuda}Comparing the system metrics for different ranking methods}
% \end{table}
% \end{center}



% \begin{center}
% \begin{table}
% \begin{tabular}{ |c|c|c| } 
%  \hline
%  method & QPS & GPU load \\ 
%  \hline
%  Float32 & 4000 & 95\% \\ 
%   \hline
%  Float16 & 6000 & 97\%\\ 
%  \hline
% Float16+MPS & 12000 & 95\%\\ 
%  \hline
% \end{tabular}
% \caption{\label{tab:qps cuda}Comparing the QPS (Query Per Second) and GPU load on single server (two T4 GPU) between different CUDA setting. Batch size = 400}
% \end{table}
% \end{center}

Finally, we compare the performance using different CUDA features. The experiments run on a GPU machine with NVIDIA T4. When running the experiments, we gradually increase the QPS from the client-side, until the more than 1\% of the server responding time begins to exceed the latency limit. We then record the current QPS as usable QPS. As shown in Table \ref{tab:qps_cuda}, the float32 version has the lowest usable QPS. Using float16 alone can decrease GPU load, but could not improve the usable QPS. Which means matrix computation is no longer the bottleneck. Combining float16 and CUDA MPS, we can double the usable QPS comparing to float32, and can fully utilize the GPU without exceeding the latency limit.


\begin{table}
  \caption{The System Performance for Different CUDA setting}
\label{tab:qps_cuda}
  \begin{tabular}{ccc}
    \toprule
 method & QPS & GPU load \\ 
    \midrule
 Float32 & 4150 & 90\% \\ 
 Float16 & 4500 & 67\%\\ 
Float16+MPS & 9400 & 100\%\\ 
  \bottomrule
\end{tabular}
\end{table}

==> model.tex <==
\section{COLD Model}
%For a long time, the design of the model and the optimization of the latency and computing power are separated, which limits the further development of the pre-ranking system. In this section, we first introduce the vector-product based method which is the previous generation of the pre-ranking model. Then we show how the co-desgin is made between the model and the computing power in COLD (Computing cost aware Online and Lightweight Deep pre-ranking system) in detail.




  
To address the problems of previous pre-ranking methods and make the co-design between model structure and computing power it costs, we propose to use FC (Fully Connected) layers and cross features in COLD, as shown in Figure \ref{cmp}. More complexly model makes it more difficult to satisfy the computing power cost constraint. 
Inspired by the SE (Squeeze-and-Excitation) block \cite{hu2018squeeze} which is firstly used in CV (Computer Vision) to explicitly model the inner-dependencies between channels, we use SE block to get the importance weights and select the most suitable features in COLD. Specifically, 
the embedding of $i_th$ input feature group is represented as $e_i$. 
The SE Block squeezes the input $e_i$ into a one-dimensional weight $s_i$, which is calculated as:
\begin{equation}
s_i = \sigma(\bm{W}e_i+\bm{b}),
\end{equation}
Where $\mathbf{W} \in \mathbb{R}^{k \times 1}, \mathbf{b} \in \mathbb{R}^{1}$.
% \begin{equation}
%  V = w * E = \text{SEBlock(E)} * E.
% \end{equation}
The weight $s$ can represent the importance of each feature group. We use the weight to rank the feature group and  select several feature groups with different top K weights as the candidate feature groups and conduct the offline test to evaluate the performance and computing power cost based on GAUC\cite{DIN}, Querys Per Seconds (QPS) and RT. Finally we choose the feature groups with the best GAUC  under the system computing power and latency constrain as our final model. In this way, the design of the model and the optimization of the computing power is not separated anymore. The trade-off between them can be conducted in a more flexible way.

The parameters of the COLD model are updated with the online learning method, which makes it more friendly to the new ads and can adapt to the newest data distribution. It is worth mentioning that the COLD can support UIC\cite{pi2019practice} to model the more complex user behaviors without increasing too much computing resources and latency. 


% the feature groups with the top k highest weights as our final features, including some user behavior features (short-term, long-term, and real-time behaviors), ad features, and context features.  As the weight of the Attention-based Gated Recurrent Unit (GRU)\cite{Cho:2014uo} layer is not in the top k list, so the structure is not in our COLD model. The final COLD model is consists of the Embedding layer and MLP layer.


% Based on the gating weight, we select the feature groups with the top k highest weights as our final features, including some user behavior features (short-term, long-term, and real-time behaviors), ad features, and context features.  As the weight of the Attention-based Gated Recurrent Unit (GRU)\cite{Cho:2014uo} layer is not in the top k list, so the structure is not in our COLD model. The final COLD model is consists of the Embedding layer and MLP layer.




==> speed.tex <==
\section{The Optimization for Inference }

\begin{figure*}[h]
\centering
\begin{minipage}[h]{0.4\textwidth}
\centering
      \includegraphics[width=0.9\textwidth] {image/row.png} 
      \caption{\label{fig:row}Row based Feature Computation. }
\end{minipage}
\begin{minipage}[h]{0.4\textwidth}
\centering
      \includegraphics[width=0.9\textwidth] {image/column.png} 
      \caption{\label{fig:column}Column based Feature Computation. }
\end{minipage}
\end{figure*}
After the design of our COLD model, it is still a challenging task to performing the inference on tens of thousands of Ads online. The computation power cost  and latency becomes  larger than the vector-based method. So we conduct several optimization on the inference pipeline. 

The real-time predicting service mainly contains two parts: feature computation and dense network computation. In feature computation, the engine pulls user and ad features from the indexing system and computes cross-features. In dense network computation, the engine will first turn features into embedding vectors and concatenate them as the input of the network. Then our optimized inference engine will perform the network forwarding pass and finally return the predicted CTR score. As latency is critical to our ad serving system, the budget for the running time of pre-ranking is very limited. The latency for computing the pre-ranking score can not be longer than 20 ms. In practice, this means we need to keep the averaging run time lower than 7ms so that the long tail queries would not affect the performance of our system. 

\subsection{Parallelism at All Level}

In order to achieve low latency inference, leveraging parallel computing is important. Our system, therefore, applies parallelism whenever is possible. Fortunately, the CTR score of the ads is independent of each other. This means they can be computed in parallel with the cost that there may be some duplicated computation related to user features. 

At a high level, one front-end user query will be split into several CTR score prediction queries. Each query handles parts of the ads and the results will be merged after all the queries return. Therefore there are trade-offs when deciding how many queries to split. More queries mean few ads for each query and therefore lower latency for an individual query. But too many queries can also lead to huge duplicated computation and system overhead. Also, as the queries are implemented using RPC (Remote Procedure Call) in our system, more queries mean more network traffic and could have a higher chance of delay or failure. In practice, we find that having 300\~ 400 ads for each query is most efficient for our cluster.

When handling each query, multi-thread processing is also used for feature computation. Again, each thread handles parts of ads to reduce the latency. And finally, when performance dense network inference, we use GPU to accelerate the computation as the most time-consuming operator of our COLD is dense matrix multiplication. 

We have been using those parallel computing techniques in our ranking system for a long time. However, they are not enough for the latency requirement of the pre-ranking model. Some specialized optimization is required.

\subsection{Column based Computation}
Traditionally, feature computation is done in a row based manner, as shown in Fig \ref{fig:row}. The ads are being processed one by one. However, such a row based method is not cache-friendly. Instead, we use a column-based method (Fig \ref{fig:column}) to put computations of one feature column together. By doing so, we are able to use techniques like SIMD (Single Instruction Multiple Data) to accelerate feature computation.

% \begin{figure*}[t]
%     \begin{center}
%       \includegraphics[width=0.3\textwidth] {dqm_paper/image/row.png} \\
%       \caption{\label{fig:row}Row based Feature Computation. }
%     \end{center}
% \end{figure*}

% \begin{figure*}[t]
%     \begin{center}
%       \includegraphics[width=0.3\textwidth] {dqm_paper/image/column.png} \\
%       \caption{\label{fig:column}Column based Feature Computation. }
%     \end{center}
% \end{figure*}






\subsection{Utilizing CUDA Features}
Even though GPU is good at accelerating deep neural networks, it is notoriously hard to fully utilize its computation power. The default implementation in open-source training frameworks like Tensorflow could result in high latency and low throughput for online inference. Such low performance is usually due to the poor arrangement of computation graph which contains unnecessary kernel launch and memory copy. Therefore, we have implemented our own inference engine which rewrites the computation graph to obtain the best performance. 

For our ranking models which contain lots of complicated units like attention and GRU, techniques like kernel fusion are already enough since the bottleneck is data movement. But for COLD, the network involves almost only dense matrix multiplication, which needs extreme optimization. 

In NVIDIA's Turing Architecture, the T4 GPU provides extreme performance for Float16 and Int8 matrix multiplication which perfectly fits our case. The theoretical peak FLOPS for float16 can be 8 times higher than float32. However, the float16 loses some precision. In practice, we found that for some scenario, as we use sum-pooling for some feature groups, the input of the dense network could be a very large number and exceed float16 representation. To solve this, one solution is to use normalization layers like the batch-norm layer. However, the BN layer itself contains moving-variance parameters whose scale could be even larger. This means the computation graph needs to be mix-precision that fully-connected layers use float16 and batch-norm layers use float32. Another approach is to use a parameter-free normalization layer. For example, the logarithmic function can easily transform large numbers into a reasonable range. However, log() function can not handle negative values and can result in a huge number when input is near zero. We, therefore, designed a piece-wised smooth function called linear-log operator to handle that unwanted behavior, as shown in Eq. \ref{eq:log}

\begin{equation}
    linear\_log(x) = \left\{
        \begin{array}{rcl}
        &-log(-x)-1   & {x< -1} \\
        &x   &  {-1\leq x\leq 1}.\\
        &log(x)+1   & {x>1}
        \end{array}
    \right.
\label{eq:log}
\end{equation}

The graphics of the linear\_log() function can be seen in Fig. \ref{fig:log}. It transforms float32 numbers into a reasonable range. So if we put a linear\_log operator in the first layer, it guarantees the input of the network would be small. Also, the linear\_log() function is $C^1$ continuous, so that it won't make network training harder. In practice, we found that after adding this layer, the network can still reach the same accuracy comparing to the original COLD.

 \begin{figure}
     \begin{center}
       \includegraphics[width=0.2\textwidth] {image/log.pdf} \\
       \caption{\label{fig:log}The linear\_log function}
     \end{center}
\end{figure}

After using float16 for inference, we found that the running time of CUDA kernel drops dramatically, and the kernel launching time becomes the bottleneck. In order to boost actual Querys Per Seconds (QPS), we further use MPS (Multi-Process Service) to reduce overhead when launching the kernels. Combining float16 and MPS, the engine throughput is twice as before.
